Variational Optimal Control for Diffusion Guidance

Sampling-time guidance and reward-based post-training act on different variables but share a core geometric objective: realizing an output-space improvement through a generative model. We organize both around a Jacobian pullback evaluated with respect to either the current noisy state or the trainable parameters. Formulating current-state conditional variational optimal control (VOC) yields Variational Optimal Guidance (VOG), which transports a terminal reward proxy into a covariance-weighted sampling correction. Under a linear-subspace denoising model, the exact pullback has no component normal to the data subspace. Distilled Variational Optimal Control (DVOC) realizes the parameter-space counterpart of this local control principle: projected reward ascent constructs a bounded endpoint displacement within a local trust region, and a sparse, forward-pinned Euler surrogate transports it to LoRA parameters. Empirically, VOG reduces DiT-XL/2 FID on ImageNet from 2.27 to 2.04 at 250 sampling steps and from 7.58 to 4.44 at 25 steps. After 20 updates on Z-Image-Turbo, DVOC improves HPSv3++ and four held-out evaluator scores over the untrained model and leads all trained comparators on these five means, while CLIP remains close to the base and DeQA declines across all trained methods. The shared pullback interface cleanly separates the desired output change from the model derivative and the actuation variable.

==> frontmatter-style.tex <==
\usepackage{tcolorbox}
\makeatletter
\definecolor{wagiblue}{rgb}{0.21,0.49,0.74}
\newcommand{\wagibanner}{%
  \noindent\begin{minipage}{\textwidth}
    \raisebox{-0.3\height}{%
      \includegraphics[height=0.27in]{fig/westlake_university_logo.png}}%
    \hspace{6pt}{\large\bfseries\color{wagiblue}Westlake AGI Lab}%
    \par\vspace{4pt}%
    {\color{wagiblue}\rule{\textwidth}{0.6pt}}%
  \end{minipage}\par
}

\newcommand{\makeagilabfrontmatter}[1]{%
  \begingroup
    \renewcommand{\encodingdefault}{T1}%
    \renewcommand{\rmdefault}{ptm}\normalfont
    \newpage\null
    \vspace*{-\baselineskip}%
    \wagibanner
    \vspace{6pt}%
    \begin{tcolorbox}[
      colback=wagiblue!4,
      colframe=wagiblue!40,
      boxrule=0.6pt,
      arc=10pt,
      left=22pt,
      right=22pt,
      top=6pt,
      bottom=6pt,
      before skip=0pt,
      after skip=0pt
    ]
    {\centering
      {\Large\bfseries\@title\par}%
      \vskip 8pt
      {\large
        \lineskip .5em
        \begin{tabular}[t]{c}
          \@author
        \end{tabular}\par
      }%
      \vskip 8pt
      {\small\@date\par}%
    }%
    \vskip 8pt
    #1%
    \end{tcolorbox}
  \endgroup
  \par\vspace{12pt}%
}

\renewenvironment{abstract}{%
  \renewcommand{\encodingdefault}{T1}%
  \renewcommand{\rmdefault}{ptm}\normalfont\small
  \centerline{\large\bfseries\abstractname}%
  \vspace{4pt}\par
  \itshape\noindent\ignorespaces
}{%
  \par
}
\makeatother

